Geometric Ultrasound Localization Microscopy

Contrast-Enhanced Ultra-Sound (CEUS) has become a viable method for non-invasive, dynamic visualization in medical diagnostics, yet Ultrasound Localization Microscopy (ULM) has enabled a revolutionary breakthrough by offering ten times higher resolution. To date, Delay-And-Sum (DAS) beamformers are used to render ULM frames, ultimately determining the image resolution capability. To take full advantage of ULM, this study questions whether beamforming is the most effective processing step for ULM, suggesting an alternative approach that relies solely on Time-Difference-of-Arrival (TDoA) information. To this end, a novel geometric framework for micro bubble localization via ellipse intersections is proposed to overcome existing beamforming limitations. We present a benchmark comparison based on a public dataset for which our geometric ULM outperforms existing baseline methods in terms of accuracy and robustness while only utilizing a portion of the available transducer data.

==> figs/img_benchmark_vertical_small.tex <==
    % https://tiborstanko.sk/closeups.html
	\begin{figure}%[H]
        \centering
		\resizebox{.85\textwidth}{!}{
			\begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
			\node[anchor=south] (FigA) at (0,0) {\includegraphics[height=3cm]{./img/gtru_ulm_img_15k_gam0.9.png}};
			\spy [closeup,magnification=1.6] on ($(FigA)+(+0.13,+0.15)$) 
			in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
			\spy [closeup,magnification=3] on ($(FigA)+(-0.235,+0.09)$) 
			in node[largewindow,anchor=east]       at ($(FigA.west)$);
			\spy [closeup,magnification=4] on ($(FigA)+(-0.175,-0.07)$) 
			in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
			\end{tikzpicture}
		}
		\caption{Ground Truth\label{fig:subfig1}}
	\end{figure}
	\begin{figure}%[H]
        \centering
		\resizebox{.85\textwidth}{!}{
			\begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
			%
			\node[anchor=south] (FigA) at (1.0,0) {\includegraphics[height=3cm]{./img/pala_ulm_img_15k_gam0.9_128chs.png}};
			\spy [closeup,magnification=1.6] on ($(FigA)+(+0.13,+0.15)$) 
			in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
			\spy [closeup,magnification=3] on ($(FigA)+(-0.235,+0.09)$) 
			in node[largewindow,anchor=east]       at ($(FigA.west)$);
			\spy [closeup,magnification=4] on ($(FigA)+(-0.175,-0.07)$) 
			in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
			\end{tikzpicture}
		}
		\caption{Radial Symmetry~\cite{heiles2022pala} from 128 transducer channels\label{fig:subfig2}}
	\end{figure}
	\begin{figure}%[H]
        \centering
		\resizebox{.85\textwidth}{!}{
			\begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
			%
			\node[anchor=south] (FigA) at (1.0,0) {\includegraphics[height=3cm]{./img/unet_ulm_img_15k_128chs_gam0.9.png}};
			\spy [closeup,magnification=1.6] on ($(FigA)+(+0.13,+0.15)$) 
			in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
			\spy [closeup,magnification=3] on ($(FigA)+(-0.235,+0.09)$) 
			in node[largewindow,anchor=east]       at ($(FigA.west)$);
			\spy [closeup,magnification=4] on ($(FigA)+(-0.175,-0.07)$) 
			in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
			\end{tikzpicture}
		}
		\caption{U-Net ULM~\cite{van2020super} from 128 transducer channels\label{fig:subfig3}}
	\end{figure}
	\begin{figure}%[H]
        \centering
		\resizebox{.85\textwidth}{!}{
			\begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
			%
			\node[anchor=south] (FigA) at (1.0,0) {\includegraphics[height=3cm]{./img/pace_ulm_img_15k_gam0.9_16chs.png}};
			\spy [closeup,magnification=1.6] on ($(FigA)+(+0.13,+0.15)$) 
			in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
			\spy [closeup,magnification=3] on ($(FigA)+(-0.235,+0.09)$) 
			in node[largewindow,anchor=east]       at ($(FigA.west)$);
			\spy [closeup,magnification=4] on ($(FigA)+(-0.175,-0.07)$) 
			in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
			\end{tikzpicture}
		}
		\caption{G-ULM (proposed) from 16 transducer channels\label{fig:subfig4}}
	\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

